Confidence Estimation and Deletion Prediction Using Bidirectional Recurrent Neural Networks

The standard approach to assess reliability of automatic speech transcriptions is through the use of confidence scores. If accurate, these scores provide a flexible mechanism to flag transcription errors for upstream and downstream applications. One challenging type of errors that recognisers make are deletions. These errors are not accounted for by the standard confidence estimation schemes and are hard to rectify in the upstream and downstream processing. High deletion rates are prominent in limited resource and highly mismatched training/testing conditions studied under IARPA Babel and Material programs. This paper looks at the use of bidirectional recurrent neural networks to yield confidence estimates in predicted as well as deleted words. Several simple schemes are examined for combination. To assess usefulness of this approach, the combined confidence score is examined for untranscribed data selection that favours transcriptions with lower deletion errors. Experiments are conducted using IARPA Babel/Material program languages.

==> abstract.tex <==
The standard approach to assess reliability of automatic speech
transcriptions is through the use of confidence scores. 
If accurate, these scores provide a flexible mechanism to flag 
transcription errors for upstream and downstream applications. 
One challenging type of errors that recognisers make are 
deletions. These errors are not accounted for by 
the standard confidence estimation schemes and are hard 
to rectify in the upstream and downstream processing. High 
deletion rates are prominent in limited resource 
and highly mismatched training/testing conditions studied 
under IARPA Babel and Material programs. 
This paper looks at the use of bidirectional recurrent neural
networks to yield confidence estimates in predicted 
as well as deleted words. A simple weighting scheme is examined 
for combination. To assess usefulness of this 
approach, the combined confidence score is examined for 
untranscribed data selection that favours transcriptions with 
lower deletion errors. Experiments are conducted using IARPA 
Babel/Material program languages.

